Dual-CLVSA: a Novel Deep Learning Approach to Predict Financial Markets with Sentiment Measurements

It is a challenging task to predict financial markets. The complexity of this task is mainly due to the interaction between financial markets and market participants, who are not able to keep rational all the time, and often affected by emotions such as fear and ecstasy. Based on the state-of-the-art approach particularly for financial market predictions, a hybrid convolutional LSTM Based variational sequence-to-sequence model with attention (CLVSA), we propose a novel deep learning approach, named dual-CLVSA, to predict financial market movement with both trading data and the corresponding social sentiment measurements, each through a separate sequence-to-sequence channel. We evaluate the performance of our approach with backtesting on historical trading data of SPDR SP 500 Trust ETF over eight years. The experiment results show that dual-CLVSA can effectively fuse the two types of data, and verify that sentiment measurements are not only informative for financial market predictions, but they also contain extra profitable features to boost the performance of our predicting system.

==> exp_result.tex <==
\section{Experiments and Results}\label{Experiments and Results}

\begin{table}
\centering
    \begin{tabular}{*{6}{c|}}
        \cline{2-6}
         & MAP & AAR & SR & DJA & YJA \\
        \hline
        \multicolumn{1}{|c|}{$LSTM_{s}^{1}$} & $42.0\%$ & $-19.9\%$ & $-1.45$ & $-0.12\%$ & $-21.3\%$  \\
        \multicolumn{1}{|c|}{$LSTM_{s}^{2}$} & $46.0\%$ & $34.2\%$ & $1.75$ & $0.24\%$ & $43.6\%$ \\
        \multicolumn{1}{|c|}{$LSTM_{s}^{3}$} & $45.5\%$ & $32.8\%$ & $1.27$ & $0.24\%$ & $41.9\%$ \\
        \multicolumn{1}{|c|}{$LSTM_{s}^{4}$} & $45.7\%$ & $28.9\%$ & $1.08$ & $0.22\%$ & $37.2\%$ \\
        \hline
        \multicolumn{1}{|c|}{$CLVSA^{1}$} & $46.1\%$ & $48.0\%$ & $2.11$ & $0.24\%$ & $57.9\%$ \\
        \multicolumn{1}{|c|}{$CLVSA^{2}$} & $45.4\%$ & $29.5\%$ & $1.10$ & $0.14\%$ & $35.6\%$ \\
        \hline
        \hline
        \multicolumn{1}{|c|}{dual-CLVSA} & \pmb{$50.7\%$}  & \pmb{$57.3\%$} & \pmb{$3.01$} & \pmb{$0.29\%$} & \pmb{$65.0\%$} \\
        \hline
    \end{tabular}
        \caption{Experimental results of SPY. MAP, AAR, SR, DJA, YJA denote the mean average precision, average annual return, and Sharpe ratio, Daily Jensen Alpha, and Yearly Jensen Alpha respectively.}
\label{tb:chpt5: result}
\end{table}

        %  $LSTM_{s}^{1}$ to $LSTM_{s}^{4}$ denote recurrent neural network with LSTM units trained and tested by historical SPY trading data, historical SPY trading data with technical indicators, historical SPY trading data with sentiment data,historical SPY trading data with technical indicators and sentiment data, respectively. $CLVSA^{1}$ and $CLVSA^{2}$ denote CLVSA trained and tested by SPY historical trading data, and SPY historical trading and SP500 TRMI data, respectively. Dual-CLVSA denotes dual-channel CLVSA trained and tested by the fusion of SPY historical trading data and SP500 TRMI data.

\subsection{Experimental results of $LSTM_{s}$}
The baseline method at the first step aims to verify the informativeness of sentiment data. We use recurrent neural network with LSTM units ($LSTM_{s}$) to train and test the following four types of datasets, SPY historical trading data, SPY historical trading data with technical indicators, SPY historical trading data with sentiment data, SPY historical trading data with technical indicators and sentiment data. We named the above four experimental sessions as $LSTM^{1}_{s}$ to $LSTM^{4}_{s}$, respectively. Table \ref{tb:chpt5: result} shows their experimental results.

Since $LSTM_{s}$ is designed for temporal feature extraction, which lacks the capability of local feature extraction. Consequently, the experimental results of $LSTM^{1}_{s}$ shows severe losses, -19.9\% average annual return (AAR). $LSTM^{2}_{s}$, however, stays positive and achieves an AAR of 34.2\%. The significant difference between the above two experiments demonstrates that technical indicators provide informative local features to $LSTM_{s}$. 

The experimental results of $LSTM^{3}_{s}$ show a positive AAR of 32.8\% as well. Although it works slightly worse than the experiment with technical indicators, the performance is significantly better than the experiment with historical SPY trading data only ($LSTM^{1}_{s}$). This result verifies that TRMI data is able to provide informative  features as technical indicators.

The experiments of $LSTM^{4}_{s}$ show interesting results. Compared to the aforementioned two experiments, the AAR drops to 28.9\%, indicating that technical indicators and TRMI data can not be fused directly although both of them contain informative features. We also observe similar results in the experiments of CLVSA with SPY historical trading data and TRMI data, which is demonstrated in the next section. 

While the experiments show  the informativeness of TRMI data, the mediocre performance of $LSTM_{s}$ with either TRMI data or the mixed data indicates that $LSTM_{s}$ may not be the optimal framework to take advantages of TRMI data.

\subsection{Experimental results of CLVSA}
The baseline method of the second step aims to reproduce the experimental results as described in \cite{ijcai2019-514} with SPY historical trading data. In \cite{ijcai2019-514}, CLVSA achieves the best performance among the five models for all the datasets of six futures. We thus test the performance of CLVSA on SPY historical trading data, named $CLVSA^{1}$, as shown in Table \ref{tb:chpt5: result}. $CLVSA^{1}$ achieves a AAR of 48.0\% over the same time period, outperforming all the previous experiments with $LSTM_{s}$. This result  verifies the superior performances of CLVSA, and also verifies CLVSA is the base model to conduct the 3rd-step experiments.

We also investigate the performance of CLVSA with a direct fusion of TRMI data and historical SPY trading data, named $CLVSA^{2}$. We treat TRMI data as alternative ``technical indicators'', in other words, TRMI data is fed into the convolutional kernels of CLVSA along with historical trading data. Similar to the experimental results of $LSTM_{s}^{4}$, $CLVSA^{2}$ underperforms $CLVSA^{2}$ for AAR by 18.5\%, which verifies again that it does not work to fuse historical trading data and TRMI data with a simple manner. 

To sum up, the first-step experiments verify that TRMI data is able to provide informative features for price movement prediction, while they also indicate that we can not simply combine TRMI data and historical trading data; the second-step experiments reproduce similar results to the ones in our previous research, verify again that CLVSA outperforms the singular models such as $LSTM_{s}$. Meanwhile, the results also show that we need a better fusion strategy to take advantages of TRMI data. 

\subsection{Experimental results of dual-CLVSA}
 Figure \ref{fig:SPY_dual_CLVSA_trmi} shows the experimental results of dual-CLVSA with the SPY TRMI data and historical trading data. The cumulative return of SPY stays positive for all the months, and eventually achieves 380\%. The monthly return stay positive for 58 out of 68 months, and no months suffer a negative return below -5\%. Daul-CLVSA also outperforms the baseline methods. Compared to $LSTM_{s}$, dual-CLVSA surpasses them for mean average precision (MAP), average annual return (AAR), Sharpe ratio (SR), Daily Jensen Alpha (DJA), and Yearly Jensen Alpha (YJA) by up to 7.3\%, 77.2\%, 4.46, 0.41\%, and 86.3\%, respectively. Compared to CLVSA, dual-CLVSA outperforms it for MAP, AAR, SR, DJA, and YJA by 1.9\%, 24.1\%, 1.30, 0.15\%, and 7.1\%, respectively. Our experimental results verify our hypothesis that with appropriate approach to fusing TRMI data and historical trading data, TRMI data provides extra informative features and thus boost the performance of the predictions and financial returns. 
 
 We explore more about how TRMI data works in dual-CLVSA with the following two cases.

 

